RIS-Enabled Localization Continuity Under Near-Field Conditions

Reconfigurable intelligent surfaces (RISs) have the potential to enable user localization in scenarios where traditional approaches fail. Building on prior work in single-antenna RIS-enabled localization, we investigate the potential to exploit wavefront curvature in geometric near-field conditions. Via a Fisher information analysis, we demonstrate that while near-field improves localization accuracy mostly at short distances when the line-of-sight (LoS) path is present, it could still provide reasonable performance when this path is blocked by relying on a single RIS reflection.

==> fig4tikz.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[scale=1\columnwidth/10cm]

\begin{axis}[%
%width=4.521in,
%height=3.563in,
width=8cm,
height=4cm,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=0.2,
xmax=30,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\norm{\vect{p}-\vect{p}_1}$ (m)},
ymode=log,
ymin=1e-04,
ymax=100,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={PEB (m)},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black},
legend pos=north west,
legend columns=2,
%legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashed,line width=1.0pt]
  table[row sep=crcr]{%
0.04	0.00186215268730394\\
0.05	0.00230263245719235\\
0.07	0.0032094588536222\\
0.1	0.00460086442514901\\
0.2	0.00932844541080264\\
0.4	0.0189713553257554\\
0.6	0.0288208326705056\\
0.8	0.038896084605726\\
1	0.0492183557465979\\
2	0.105798656086568\\
4	0.268229887066295\\
6	0.599180131294855\\
8	1.32399691487287\\
10	2.74494773703343\\
20	31.3495240212605\\
25	67.3474968119524\\
30	124.241712295786\\
};
\addlegendentry{\small{$32\times 32$, LOS, FF}}

\addplot [color=red,line width=1.0pt]
  table[row sep=crcr]{%
0.04	3.73131355937637e-06\\
0.05	4.91222010310085e-06\\
0.06	6.37903836681992e-06\\
0.07	8.16967749544015e-06\\
0.08	1.03256846954514e-05\\
0.0900000000000001	1.28904101147387e-05\\
0.1	1.59099175404481e-05\\
0.2	8.16343032713815e-05\\
0.4	0.000558878364386224\\
0.6	0.00182366918704667\\
1	0.00820199436121272\\
2	0.0560423812205703\\
4	0.23911604830285\\
6	0.567885497770013\\
8	1.26326670466584\\
10	2.60422741151986\\
15	10.5705172177666\\
20	28.3096432290842\\
25	59.6739388438501\\
30	108.465037993349\\
};
\addlegendentry{\small{$32\times 32$,  LOS, NF}}

\addplot [color=green, dashdotted,line width=1.0pt]
  table[row sep=crcr]{%
0.04	0.000931065201455121\\
0.05	0.00115114366554768\\
0.07	0.00160477514012448\\
0.1	0.00230040217328665\\
0.2	0.0046642737293539\\
0.4	0.00948508200507767\\
0.6	0.0144101010469822\\
0.8	0.0194465801047027\\
1	0.0246077761131366\\
2	0.0528940145709707\\
4	0.134078100883869\\
6	0.299492935166486\\
8	0.661787618969598\\
10	1.37211108739385\\
20	15.672081662244\\
25	33.6682405074706\\
30	62.1112249837932\\
};
\addlegendentry{\small{$64\times 64$, LOS, FF}}





\addplot [color=green,line width=1.0pt]
  table[row sep=crcr]{%
0.04	1.84986183027158e-06\\
0.05	2.19564573319776e-06\\
0.06	2.59238769037705e-06\\
0.07	3.04103961690329e-06\\
0.08	3.54471453843693e-06\\
0.0900000000000001	4.10755920750831e-06\\
0.1	4.73411101079389e-06\\
0.2	1.56641857052958e-05\\
0.4	8.1055278470184e-05\\
0.6	0.000245097093685697\\
0.8	0.00055694696503344\\
1	0.00106554960764821\\
2	0.008199750645326\\
4	0.0591698594957373\\
6	0.178475393968789\\
8	0.412039767116876\\
10	0.82279584756329\\
15	2.9653187866377\\
20	7.28129153161015\\
30	25.3362298773395\\
};
\addlegendentry{\small{$64\times 64$, LOS, NF}}

\addplot [color=blue, dashed, line width=1.0pt]%mark=*, mark options={solid, blue}]
  table[row sep=crcr]{%
0.04	0.00046551771320694\\
0.05	0.000575587205706267\\
0.06	0.00068823404437399\\
0.07	0.000802419622497375\\
0.0799999999999999	0.000917668722989392\\
0.09	0.00103366893096305\\
0.1	0.00115023457036062\\
0.2	0.00233212543877342\\
0.4	0.00474257732000456\\
0.6	0.00720499020364342\\
0.8	0.00972325138469318\\
1	0.0123037899491414\\
2	0.0264464132372998\\
4	0.0670350999908505\\
6	0.149734374200282\\
8	0.330869165863359\\
10	0.686009453218745\\
15	2.85639573868134\\
20	7.83568813151138\\
25	16.8326617227404\\
30	31.0579801746014\\
};
\addlegendentry{\small{$128\times128$, LOS, FF}}

\addplot [color=blue,line width=1.0pt]
  table[row sep=crcr]{%
0.04	1.17295620522205e-06\\
0.05	1.3041052175807e-06\\
0.06	1.44828677147416e-06\\
0.07	1.60333764948404e-06\\
0.08	1.76865585948422e-06\\
0.0900000000000001	1.94425754928126e-06\\
0.1	2.13046267441015e-06\\
0.2	4.68946785907192e-06\\
0.4	1.56031538185567e-05\\
0.6	3.90010366223906e-05\\
0.8	8.0911044966818e-05\\
1	0.000147466906062466\\
2	0.00106489371331089\\
6	0.0273828489139322\\
10	0.12639962036192\\
30	3.44615377681013\\
};
\addlegendentry{\small{$128\times 128$, LOS, NF}}

\end{axis}


\end{tikzpicture}%

==> fig5tikz.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}[scale=1\columnwidth/10cm]

\begin{axis}[%
%width=4.521in,
%height=3.563in,
width=8cm,
height=4cm,
at={(1.011in,0.642in)},
%at={(0.758in,0.484in)},
scale only axis,
xmode=log,
xmin=0.2,
xmax=30,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\norm{\vect{p}-\vect{p}_1}$ (m)},
ymode=log,
ymin=1e-4,
ymax=100,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={PEB (m)},
axis background/.style={fill=white},
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1,line width=1.0pt]
  table[row sep=crcr]{%
0.04	3.73131355937637e-06\\
0.05	4.91222010310085e-06\\
0.06	6.37903836681992e-06\\
0.07	8.16967749544015e-06\\
0.08	1.03256846954514e-05\\
0.0900000000000001	1.28904101147387e-05\\
0.1	1.59099175404481e-05\\
0.2	8.16343032713815e-05\\
0.4	0.000558878364386224\\
0.6	0.00182366918704667\\
1	0.00820199436121272\\
2	0.0560423812205703\\
4	0.23911604830285\\
6	0.567885497770013\\
8	1.26326670466584\\
10	2.60422741151986\\
15	10.5705172177666\\
20	28.3096432290842\\
25	59.6739388438501\\
30	108.465037993349\\
};
\addlegendentry{\small{$32\times 32$, LOS, NF}}

\addplot [color=red,line width=1.0pt]
  table[row sep=crcr]{%
0.04	3.73116048030168e-06\\
0.05	4.91201047220193e-06\\
0.06	6.37901172015407e-06\\
0.07	8.16952965952151e-06\\
0.08	1.03252289327342e-05\\
0.0900000000000001	1.28901743445148e-05\\
0.1	1.59099623818101e-05\\
0.2	8.16357213374988e-05\\
0.4	0.000559088049137686\\
0.6	0.00182721710175131\\
1	0.0083171240051914\\
4	0.527483236482584\\
25	128.703682513473\\
};
\addlegendentry{\small{$32\times 32$, NLOS, NF}}

\addplot [color=red, dashdotted,line width=1.0pt]
  table[row sep=crcr]{%
0.04	1.84985733909999e-06\\
0.05	2.19563674424356e-06\\
0.06	2.59237813165439e-06\\
0.07	3.04102720821578e-06\\
0.08	3.54471612545913e-06\\
0.0900000000000001	4.10753929597977e-06\\
0.1	4.73409939223748e-06\\
0.2	1.56642449557332e-05\\
0.4	8.10575664476211e-05\\
0.6	0.000245127836577353\\
0.8	0.000557166600392192\\
1	0.00106651333207966\\
2	0.00829958968745062\\
8	0.526507075894715\\
30	27.7497679586943\\
};
\addlegendentry{\small{$64\times 64$, NLOS, NF}}

\end{axis}

\end{tikzpicture}%
